Entropic Descent Archetypal Analysis for Blind Hyperspectral Unmixing

In this paper, we introduce a new algorithm based on archetypal analysis for blind hyperspectral unmixing, assuming linear mixing of endmembers. Archetypal analysis is a natural formulation for this task. This method does not require the presence of pure pixels (i.e., pixels containing a single material) but instead represents endmembers as convex combinations of a few pixels present in the original hyperspectral image. Our approach leverages an entropic gradient descent strategy, which (i) provides better solutions for hyperspectral unmixing than traditional archetypal analysis algorithms, and (ii) leads to efficient GPU implementations. Since running a single instance of our algorithm is fast, we also propose an ensembling mechanism along with an appropriate model selection procedure that make our method robust to hyper-parameter choices while keeping the computational complexity reasonable. By using six standard real datasets, we show that our approach outperforms state-of-the-art matrix factorization and recent deep learning methods. We also provide an open-source PyTorch implementation: https://github.com/inria-thoth/EDAA.

==> tables/summary.tex <==
% \begin{tabular}{c | c | c c c c c c c}
%   \toprule
%   & & FCLSU & NMF-QMV & AA & RAA & CNNAEU & MiSiCNet & EDAA \\
%   \hline
%   \multirow{4}{*}{Samson}
%   & Soil & 11.28 & 13.67 & 6.16 & 6.02 & 25.82 & 18.18 & \textbf{5.91} \\
%   & Tree & 9.13 & 8.4 & 4.00 & 4.12 & 22.88 & 17.91 & \textbf{3.84} \\
%   & Water & 5.05 & 11.61 & 2.30 & \textbf{2.08} & 25.32 & 31.30 & 2.73\\
%   \cline{2-9}
%   & Overall & 8.88 & 11.44 & 4.44 & 4.38 & 25.18 & 23.32 & \textbf{4.36}\\
%   \hline
%   \hline
%   \multirow{5}{*}{Jasper Ridge}
%   & Dirt & 21.23 & 19.97 & 10.24 & 10.54 & 38.42 & 22.11 & \textbf{8.10} \\
%   & Road & 24.72 & 26.13 & 9.79 & 8.75 & 31.22 & 24.89 & \textbf{7.84} \\
%   & Tree & 11.20 & 14.55 & \textbf{6.32} & 9.87 & 27.82 & 9.57 & 7.76 \\
%   & Water & 13.61 & 19.81 & 6.77 & \textbf{5.00} & 21.28 & 11.44 & 5.66 \\
%   \cline{2-9}
%   & Overall & 18.52 & 20.53 & 8.46 & 8.81 & 30.75 & 18.24 & \textbf{7.41} \\
%   \hline
%   \hline
%   \multirow{5}{*}{Urban4}
%   & Road & 30.54 & 20.25 & 11.12 & \textbf{8.80} & 26.74 & 37.69 & 13.00 \\
%   & Grass & 32.99 & 20.22 & 11.55 & 11.29 & 30.53 & 31.64 & \textbf{9.55} \\
%   & Roof & 15.40 & 13.29 & 7.28 & \textbf{5.31} & 20.24 & 15.63 & 8.21 \\
%   & Tree & 20.02 & 21.56 & 8.62 & 8.41 & 21.33 & 24.52 & \textbf{6.96} \\
%   \cline{2-9}
%   & Overall & 25.78 & 19.11 & 9.80 & \textbf{8.71} & 25.22 & 28.58 & 9.70\\
%   \hline
%   \hline
%   \multirow{7}{*}{Urban6}
%   & Road & 31.61 & 24.81 & 19.23 & 19.97 & 27.86 & 19.32 & \textbf{13.63} \\
%   & Grass & 23.62 & 27.97 & \textbf{9.73} & 27.02 & 36.36 & 25.67 & 10.05 \\
%   & Roof & 13.00 & 16.39 & 10.92 & \textbf{5.89} & 13.36 & 13.76 & 9.22 \\
%   & Tree & 16.14 & 19.95 & 14.45 & 20.07 & 22.41 & 24.53 &\textbf{8.79} \\
%   & Dirt & 25.06 & 24.31 & 27.76 & 24.82 & 29.27 & 15.58 & \textbf{9.70} \\
%   & Metal & \textbf{12.99} & 13.40 & 17.53 & 19.22 & 26.11 & 33.67 & 19.25 \\
%   \cline{2-9}
%   & Overall & 21.54 & 21.74 & 17.66 & 20.62 & 27.25 & 23.09 & \textbf{12.34} \\
%   \hline
%   \hline
%   \multirow{5}{*}{APEX}
%   & Road & 33.31 & 31.43 & 34.12 & 35.68 & 35.34 & 13.67 & \textbf{13.12} \\
%   & Tree & 20.97 & 24.62 & 22.49 & 24.61 & 14.29 & 14.92 & \textbf{14.13} \\
%   & Roof & 14.15 & 14.73 & 18.54 & 19.81 & 28.29 & \textbf{11.38} & 11.79 \\
%   & Water & 18.03 & 17.99 & 16.90 & \textbf{16.85} & 35.40 & 19.84 & 16.95 \\
%   \cline{2-9}
%   & Overall & 22.77 & 23.10 & 23.98 & 25.27 & 24.10 & 15.27 & \textbf{14.13} \\
%   \hline
%   \hline
%   \multirow{7}{*}{WDC}
%   & Grass & 30.90 & 34.69 & 31.92 & 31.03 & 43.05 & \textbf{24.51} & 31.75 \\
%   & Tree & 22.42 & 19.90 & 20.13 & 15.96 & 35.03 & \textbf{10.55} & 11.08 \\
%   & Road & 27.90 & 22.49 & 38.87 & 35.42 & 28.57 & 18.16 & \textbf{9.48} \\
%   & Roof & \textbf{8.71} & 19.81 & 20.89 & 20.45 & 23.92 & 18.88 & 33.99 \\
%   & Water & 17.76 & 20.34 & 14.06 & 14.00 & 36.17 & 18.02 & \textbf{9.96} \\
%   & Trail & 12.80 & 12.36 & 15.24 & 15.92 & 28.40 & 9.66 & \textbf{7.29} \\
%   \cline{2-9}
%   & Overall & 21.57 & 22.60 & 25.17 & 23.59 & 33.59 & \textbf{17.40} & 20.53\\
%   \bottomrule
% \end{tabular}

% \begin{tabular}{c | c | c c c c c c c}
%   \toprule
%   & & FCLSU & CNNAEU & MiSiCNet & NMF-QMV & AA & RAA & EDAA \\
%   \hline
%   \multirow{4}{*}{Samson}
%   & Soil & 11.28 & 25.82 & 18.18 & 13.67 & 6.16 & 6.02 & \textbf{5.91} \\
%   & Tree & 9.13 & 22.88 & 17.91 & 8.4 & 4.00 & 4.12 & \textbf{3.84} \\
%   & Water & 5.05 & 25.32 & 31.30 & 11.61 & 2.30 & \textbf{2.08} & 2.73\\
%   \cline{2-9}
%   & Overall & 8.88 & 25.18 & 23.32 & 11.44 & 4.44 & 4.38 & \textbf{4.36}\\
%   \hline
%   \hline
%   \multirow{5}{*}{Jasper Ridge}
%   & Dirt & 21.23 & 38.42 & 22.11 & 19.97 & 10.24 & 10.54 & \textbf{8.10} \\
%   & Road & 24.72 & 31.22 & 24.89 & 26.13 & 9.79 & 8.75 & \textbf{7.84} \\
%   & Tree & 11.20 & 27.82 & 9.57 & 14.55 & \textbf{6.32} & 9.87 & 7.76 \\
%   & Water & 13.61 & 21.28 & 11.44 & 19.81 & 6.77 & \textbf{5.00} & 5.66 \\
%   \cline{2-9}
%   & Overall & 18.52 & 30.75 & 18.24 & 20.53 & 8.46 & 8.81 & \textbf{7.41} \\
%   \hline
%   \hline
%   \multirow{5}{*}{Urban4}
%   & Road & 30.54 & 26.74 & 37.69 & 20.25 & 11.12 & \textbf{8.80} & 13.00 \\
%   & Grass & 32.99 & 30.53 & 31.64 & 20.22 & 11.55 & 11.29 & \textbf{9.55} \\
%   & Roof & 15.40 & 20.24 & 15.63 & 13.29 & 7.28 & \textbf{5.31} & 8.21 \\
%   & Tree & 20.02 & 21.33 & 24.52 & 21.56 & 8.62 & 8.41 & \textbf{6.96} \\
%   \cline{2-9}
%   & Overall & 25.78 & 25.22 & 28.58 & 19.11 & 9.80 & \textbf{8.71} & 9.70\\
%   \hline
%   \hline
%   \multirow{7}{*}{Urban6}
%   & Road & 31.61 & 27.86 & 19.32 & 24.81 & 19.23 & 19.97 & \textbf{13.63} \\
%   & Grass & 23.62 & 36.36 & 25.67 & 27.97 & \textbf{9.73} & 27.02 & 10.05 \\
%   & Roof & 13.00 & 13.36 & 13.76 & 16.39 & 10.92 & \textbf{5.89} & 9.22 \\
%   & Tree & 16.14 & 22.41 & 24.53 & 19.95 & 14.45 & 20.07 &\textbf{8.79} \\
%   & Dirt & 25.06 & 29.27 & 15.58 & 24.31 & 27.76 & 24.82 & \textbf{9.70} \\
%   & Metal & \textbf{12.99} & 26.11 & 33.67 & 13.40 & 17.53 & 19.22 & 19.25 \\
%   \cline{2-9}
%   & Overall & 21.54 & 27.25 & 23.09 & 21.74 & 17.66 & 20.62 & \textbf{12.34} \\
%   \hline
%   \hline
%   \multirow{5}{*}{APEX}
%   & Road & 33.31 & 35.34 & 13.67 & 31.43 & 34.12 & 35.68 & \textbf{13.12} \\
%   & Tree & 20.97 & 14.29 & 14.92 & 24.62 & 22.49 & 24.61 & \textbf{14.13} \\
%   & Roof & 14.15 & 28.29 & \textbf{11.38} & 14.73 & 18.54 & 19.81 & 11.79 \\
%   & Water & 18.03 & 35.40 & 19.84 & 17.99 & 16.90 & \textbf{16.85} & 16.95 \\
%   \cline{2-9}
%   & Overall & 22.77 & 24.10 & 15.27 & 23.10 & 23.98 & 25.27 & \textbf{14.13} \\
%   \hline
%   \hline
%   \multirow{7}{*}{WDC}
%   & Grass & 30.90 & 43.05 & \textbf{24.51} & 34.69 & 31.92 & 31.03 & 31.75 \\
%   & Tree & 22.42 & 35.03 & \textbf{10.55} & 19.90 & 20.13 & 15.96 & 11.08 \\
%   & Road & 27.90 & 28.57 & 18.16 & 22.49 & 38.87 & 35.42 & \textbf{9.48} \\
%   & Roof & \textbf{8.71} & 23.92 & 18.88 & 19.81 & 20.89 & 20.45 & 33.99 \\
%   & Water & 17.76 & 36.17 & 18.02 & 20.34 & 14.06 & 14.00 & \textbf{9.96} \\
%   & Trail & 12.80 & 28.40 & 9.66 & 12.36 & 15.24 & 15.92 & \textbf{7.29} \\
%   \cline{2-9}
%   & Overall & 21.57 & 33.59 & \textbf{17.40} & 22.60 & 25.17 & 23.59 & 20.53\\
%   \bottomrule
% \end{tabular}
% \begin{tabular}{c | c | c c c c c c c}
%   \toprule
%   & & FCLSU \cite{nascimento_vertex_2005, heinz_fully_2001} & CNNAEU \cite{palsson_convolutional_2021} & MiSiCNet \cite{rasti_misicnet_2022} & NMF-QMV \cite{zhuang_regularization_2019} & AA & RAA & EDAA \\
%   \hline
%   \multirow{4}{*}{Samson}
%   & Soil & 11.28 & 45.23 & 6.47 & 13.67 & 6.16 & \underline{6.02} & \textbf{5.91} \\
%   & Tree & 9.13 & 45.83 & 5.38 & 8.4 & \underline{4.00} & 4.12 & \textbf{3.84} \\
%   & Water & 5.05 & 18.78 & 3.47 & 11.61 & \underline{2.30} & \textbf{2.08} & 2.73\\
%   \cline{2-9}
%   & Overall & 8.88 & 39.02 & 5.25 & 11.44 & 4.44 & \underline{4.38} & \textbf{4.36}\\
%   \hline
%   \hline
%   \multirow{5}{*}{Jasper Ridge}
%   & Dirt & 21.23 & 38.17 & 21.68 & 19.97 & \underline{10.24} & 10.54 & \textbf{8.10} \\
%   & Road & 24.72 & 43.87 & 24.94 & 26.13 & 9.79 & \underline{8.75} & \textbf{7.84} \\
%   & Tree & 11.20 & 32.93 & \textbf{3.41} & 14.55 & \underline{6.32} & 9.87 & 7.76 \\
%   & Water & 13.61 & 28.28 & 7.07 & 19.81 & 6.77 & \textbf{5.00} & \underline{5.66} \\
%   \cline{2-9}
%   & Overall & 18.52 & 37.83 & 16.98 & 20.53 & \underline{8.46} & 8.81 & \textbf{7.41} \\
%   \hline
%   \hline
%   \multirow{5}{*}{Urban4}
%   & Road & 30.54 & 38.22 & \underline{10.30} & 20.25 & 11.12 & \textbf{8.80} & 13.00 \\
%   & Grass & 32.99 & 49.72 & 12.35 & 20.22 & 11.55 & \underline{11.29} & \textbf{9.55} \\
%   & Roof & 15.40 & 25.15 & 8.01 & 13.29 & \underline{7.28} & \textbf{5.31} & 8.21 \\
%   & Tree & 20.02 & 41.04 & 8.78 & 21.56 & 8.62 & \underline{8.41} & \textbf{6.96} \\
%   \cline{2-9}
%   & Overall & 25.78 & 40.14 & 10.00 & 19.11 & 9.80 & \textbf{8.71} & \underline{9.70}\\
%   \hline
%   \hline
%   \multirow{7}{*}{Urban6}
%   & Road & 31.61 & 31.43 & \underline{19.18} & 24.81 & 19.23 & 19.97 & \textbf{13.63} \\
%   & Grass & 23.62 & 49.55 & 18.84 & 27.97 & \textbf{9.73} & 27.02 & \underline{10.05} \\
%   & Roof & 13.00 & 21.81 & \underline{7.41} & 16.39 & 10.92 & \textbf{5.89} & 9.22 \\
%   & Tree & 16.14 & 34.99 & \underline{11.72} & 19.95 & 14.45 & 20.07 &\textbf{8.79} \\
%   & Dirt & 25.06 & 59.12 & \underline{23.95} & 24.31 & 27.76 & 24.82 & \textbf{9.70} \\
%   & Metal & \textbf{12.99} & 26.85 & 33.67 & \underline{13.40} & 17.53 & 19.22 & 19.25 \\
%   \cline{2-9}
%   & Overall & 21.54 & 41.17 & \underline{16.27} & 21.74 & 17.66 & 20.62 & \textbf{12.34} \\
%   \hline
%   \hline
%   \multirow{5}{*}{APEX}
%   & Road & 33.31 & 36.42 & 32.66 & \underline{31.43} & 34.12 & 35.68 & \textbf{13.12} \\
%   & Tree & 20.97 & 39.99 & \underline{19.97} & 24.62 & 22.49 & 24.61 & \textbf{14.13} \\
%   & Roof & \underline{14.15} & 32.69 & 18.42 & 14.73 & 18.54 & 19.81 & \textbf{11.79} \\
%   & Water & 18.03 & 32.32 & \underline{16.88} & 17.99 & 16.90 & \textbf{16.85} & 16.95 \\
%   \cline{2-9}
%   & Overall & \underline{22.77} & 35.76 & 22.86 & 23.10 & 23.98 & 25.27 & \textbf{14.13} \\
%   \hline
%   \hline
%   \multirow{7}{*}{WDC}
%   & Grass & \textbf{30.90} & 46.77 & 31.61 & 34.69 & 31.92 & \underline{31.03} & 31.75 \\
%   & Tree & 22.42 & 36.06 & 23.64 & 19.90 & 20.13 & \underline{15.96} & \textbf{11.08} \\
%   & Road & 27.90 & 34.64 & 34.91 & \underline{22.49} & 38.87 & 35.42 & \textbf{9.48} \\
%   & Roof & \textbf{8.71} & 14.84 & \underline{11.98} & 19.81 & 20.89 & 20.45 & 33.99 \\
%   & Water & 17.76 & 40.24 & 14.72 & 20.34 & 14.06 & \underline{14.00} & \textbf{9.96} \\
%   & Trail & 12.80 & 23.17 & \underline{12.07} & 12.36 & 15.24 & 15.92 & \textbf{7.29} \\
%   \cline{2-9}
%   & Overall & \underline{21.57} & 35.64 & 23.39 & 22.60 & 25.17 & 23.59 & \textbf{20.53}\\
%   \bottomrule
% \end{tabular}

% \begin{tabular}{c | c | c c c c c c c}
%   \toprule
%   & & FCLSU \cite{nascimento_vertex_2005, heinz_fully_2001} & Endnet \cite{ozkan_endnet_2018} & MiSiCNet \cite{rasti_misicnet_2022} & NMF-QMV \cite{zhuang_regularization_2019} & AA & RAA & EDAA \\
%   \hline
%   \multirow{4}{*}{Samson}
%   & Soil & 11.28 & 11.61 & 6.47 & 13.67 & 6.16 & \underline{6.02} & \textbf{5.74} \\
%   & Tree & 9.13 & 7.72 & 5.38 & 8.4 & \underline{4.00} & 4.12 & \textbf{3.77} \\
%   & Water & 5.05 & 6.86 & 3.47 & 11.61 & \underline{2.30} & \textbf{2.08} & 2.59\\
%   \cline{2-9}
%   & Overall & 8.88 & 8.97 & 5.25 & 11.44 & 4.44 & \underline{4.38} & \textbf{4.24}\\
%   \hline
%   \hline
%   \multirow{5}{*}{Jasper Ridge}
%   & Dirt & 21.23 & 18.26 & 21.68 & 19.97 & \underline{10.24} & 10.54 & \textbf{7.32} \\
%   & Road & 24.72 & 29.40 & 24.94 & 26.13 & 9.79 & \underline{8.75} & \textbf{7.61} \\
%   & Tree & 11.20 & 4.00 & \textbf{3.41} & 14.55 & \underline{6.32} & 9.87 & 6.63 \\
%   & Water & 13.61 & 22.38 & 7.07 & 19.81 & 6.77 & \textbf{5.00} & \underline{5.69} \\
%   \cline{2-9}
%   & Overall & 18.52 & 20.70 & 16.98 & 20.53 & \underline{8.46} & 8.81 & \textbf{6.85} \\
%   \hline
%   \hline
%   \multirow{5}{*}{Urban4}
%   & Road & 30.54 & 12.04 & 10.30 & 20.25 & 11.12 & \underline{8.80} & \textbf{8.62} \\
%   & Grass & 32.99 & 17.94 & 12.35 & 20.22 & 11.55 & \underline{11.29} & \textbf{9.28} \\
%   & Roof & 15.40 & 11.28 & 8.01 & 13.29 & 7.28 & \textbf{5.31} & \underline{6.37} \\
%   & Tree & 20.02 & 11.69 & 8.78 & 21.56 & 8.62 & \underline{8.41} & \textbf{6.27} \\
%   \cline{2-9}
%   & Overall & 25.78 & 13.52 & 10.00 & 19.11 & 9.80 & \underline{8.71} & \textbf{7.75}\\
%   \hline
%   \hline
%   \multirow{7}{*}{Urban6}
%   & Road & 31.61 & \underline{17.44} & 19.18 & 24.81 & 19.23 & 19.97 & \textbf{11.39} \\
%   & Grass & 23.62 & 31.47 & 18.84 & 27.97 & \textbf{9.73} & 27.02 & \underline{18.61} \\
%   & Roof & 13.00 & 9.35 & 7.41 & 16.39 & 10.92 & \textbf{5.89} & \underline{6.01} \\
%   & Tree & 16.14 & 15.50 & \underline{11.72} & 19.95 & 14.45 & 20.07 &\textbf{9.85} \\
%   & Dirt & 25.06 & 30.67 & \underline{23.95} & 24.31 & 27.76 & 24.82 & \textbf{15.94} \\
%   & Metal & \textbf{12.99} & 25.21 & 33.67 & \underline{13.40} & 17.53 & 19.22 & 15.86 \\
%   \cline{2-9}
%   & Overall & 21.54 & 23.09 & \underline{16.27} & 21.74 & 17.66 & 20.62 & \textbf{13.63} \\
%   \hline
%   \hline
%   \multirow{5}{*}{APEX}
%   & Road & 33.31 & \underline{29.32} & 32.66 & 31.43 & 34.12 & 35.68 & \textbf{16.54} \\
%   & Tree & 20.97 & \underline{18.18} & 19.97 & 24.62 & 22.49 & 24.61 & \textbf{14.48} \\
%   & Roof & \underline{14.15} & 15.88 & 18.42 & 14.73 & 18.54 & 19.81 & \textbf{11.27} \\
%   & Water & 18.03 & 17.47 & 16.88 & 17.99 & 16.90 & \underline{16.85} & \textbf{16.83} \\
%   \cline{2-9}
%   & Overall & 22.77 & \underline{20.90} & 22.86 & 23.10 & 23.98 & 25.27 & \textbf{14.94} \\
%   \hline
%   \hline
%   \multirow{7}{*}{WDC}
%   & Grass & \underline{30.90} & \textbf{27.35} & 31.61 & 34.69 & 31.92 & 31.03 & 32.53 \\
%   & Tree & 22.42 & 35.98 & 23.64 & 19.90 & 20.13 & \underline{15.96} & \textbf{11.46} \\
%   & Road & 27.90 & 38.49 & 34.91 & \underline{22.49} & 38.87 & 35.42 & \textbf{13.97} \\
%   & Roof & \textbf{8.71} & 27.04 & \underline{11.98} & 19.81 & 20.89 & 20.45 & 29.31 \\
%   & Water & 17.76 & \underline{12.94} & 14.72 & 20.34 & 14.06 & 14.00 & \textbf{9.63} \\
%   & Trail & 12.80 & 12.63 & \textbf{12.07} & \underline{12.36} & 15.24 & 15.92 & 13.19 \\
%   \cline{2-9}
%   & Overall & \underline{21.57} & 27.64 & 23.39 & 22.60 & 25.17 & 23.59 & \textbf{20.46}\\
%   \bottomrule
% \end{tabular}

% Remove RAA

\begin{tabular}{c | c | c c c c c c}
  \toprule
  & & FCLSU \cite{nascimento_vertex_2005, heinz_fully_2001} & Endnet \cite{ozkan_endnet_2018} & MiSiCNet \cite{rasti_misicnet_2022} & NMF-QMV \cite{zhuang_regularization_2019} & AA & EDAA \\
  \hline
  \multirow{2}{*}{Samson}
  & RMSE & 8.88 & 8.97 & 5.25 & 11.44 & \underline{4.44} & \textbf{4.24}\\
  & SAD & 4.32 & \underline{1.34} & 3.32 & 7.13 & \textbf{1.32} & 1.64\\
  \hline
  \multirow{2}{*}{Jasper Ridge}
  & RMSE & 18.52 & 20.70 & 16.98 & 20.53 & \underline{8.46} & \textbf{6.85} \\
  & SAD & 19.46 & 9.77 & 7.44 & 21.77 & \underline{4.52} & \textbf{3.22} \\
  \hline
  \multirow{2}{*}{Urban4}
  & RMSE & 25.78 & 13.52 & 10.00 & 19.11 & \underline{9.80} & \textbf{7.75}\\
  & SAD & 26.74 & \textbf{3.89} & 8.07 & 22.42 & 6.16 & \underline{5.36} \\
  \hline
  \multirow{2}{*}{Urban6}
  & RMSE & 21.54 & 23.09 & \underline{16.27} & 21.74 & 17.66 & \textbf{13.63} \\
  & SAD & 30.21 & \underline{9.56} & 11.95 & 29.90 & 15.14 & \textbf{8.64} \\
  \hline
  \multirow{2}{*}{APEX}
  & RMSE & 22.77 & \underline{20.90} & 22.86 & 23.10 & 23.98 & \textbf{14.94} \\
  & SAD & 17.44 & \underline{7.30} & 13.38 & 22.07 & 13.21 & \textbf{6.06} \\
  \hline
  \multirow{2}{*}{WDC}
  & RMSE & \underline{21.57} & 27.64 & 23.39 & 22.60 & 25.17 & \textbf{20.46}\\
  & SAD & 20.54 & \textbf{10.02} & 16.11 & 23.93 & 18.68 & \underline{12.40}\\
  \bottomrule
\end{tabular}

